Repairing mappings under policy views

The problem of data exchange involves a source schema, a target schema and a set of mappings from transforming the data between the two schemas. We study the problem of data exchange in the presence of privacy restrictions on the source. The privacy restrictions are expressed as a set of policy views representing the information that is safe to expose over all instances of the source. We propose a protocol that provides formal privacy guarantees and is data-independent, i.e., if certain criteria are met, then the protocol guarantees that the mappings leak no sensitive information independently of the data that lies in the source. We also propose an algorithm for repairing an input mapping w.r.t. a set of policy views, in cases where the input mapping leaks sensitive information. The empirical evaluation of our work shows that the proposed algorithm is quite efficient, repairing sets of 300 s-t tgds in an average time of 5s on a commodity machine. To the best of our knowledge, our work is the first one that studies the problems of exchanging data and repairing mappings under such privacy restrictions. Furthermore, our work is the first to provide practical algorithms for a logical privacy-preservation paradigm, described as an open research challenge in previous work on this area.

==> learning.tex <==
\section{Learning the user preferences} \label{sec:learning}

In the above presentation of the repairing algorithm, we have assumed 
that $\pref$ is fixed. Such an assumption is reasonable if the
preference mechanism is hardcoded, i.e., if we know that the s-t tgd
with highest number of exported variables is chosen at each iteration.  
In this section, we explain how this function can be learned by
relying on off-the-shelf machine learning algorithms and based on training
sets in which former user choices have been recorded.  

In order to be able to rank the possible repairs and use inference on
previously specified user's choices, we first need to define suitable metrics for comparing 
each pair of repairs $\mu_{r_1}$ and $\mu_{r_2}$ for a given s-t tgd $\mu$.
In case the number of possible repairs for $\mu$ is greater than two, the metrics will compare the 
repairs pair by pair. 
For instance, Example~\ref{example:frepair} presents three different repairs for the s-t tgd $\mu_1$.
Since our algorithm modifies the exported and the repeated variables in the bodies of the s-t tgds, 
we ground our metrics on the following two parameters: $\Delta_{FV}$ amounting to the difference 
between the number of exported variables in $\mu_{r_1}$ and $\mu_{r_2}$, 
and $\Delta_J$ corresponding to the difference 
between the number of joins in the bodies of $\mu_{r_1}$ and $\mu_{r_2}$.

The key intuition behind applying statistical learning to rank possible safe rewritings of s-t tgds is to leverage an available training set of correctly identified observations. Each observation consists of the two metrics $\Delta_{FV}$ and $\Delta_{J}$ defined above along with the s-t tgd that better fits the values $\Delta_{FV}$ and $\Delta_{J}$. 
More formally, we define a vector of variables ${\mathbf{X} = \langle \Delta_{FV},\Delta_{J} \rangle}$ 
and we use it as input to train the learning model. 
We define a qualitative output $G$ embodying the s-t tgd $\mu_{r_1}$ and $\mu_{r_2}$ chosen by the preference function $\pref$.
We next denote by ${\langle \delta_{FV},\delta_{J} \rangle}$ the observed values of the vector $\mathbf{X}$
and by $g$ the actual value of the qualitative output $G$.
Let $\hat{G}$ be the prediction associated to $G$ obtained by the learning model. 
The goal of the learning model is to obtain, for each observation ${\langle \delta_{FV},\delta_{J} \rangle}$ of $\mathbf{X}$,
a predicted value $\hat{g}$ of $\hat{G}$ that fits the ground-truth value $g$ corresponding to 
${\langle \delta_{FV},\delta_{J} \rangle}$. 

We employ the k-NN classification algorithm \cite{friedman2001elements} as the supervised learning
method for learning $\pref$. This algorithm has been chosen due to its flexibility in comparing a new 
item to classify with the existing items in the training set, which are the k-nearest to the former in terms of their similarity. 

In our setting, training sets consist of measurements $\{(\langle \delta_{FV,i},\delta_{J,i} \rangle,g_i) | i=1,\dots,N \}$, such that
${\langle \delta_{FV,i},\delta_{J,i} \rangle}$ are values of $\mathbf{X}$ on the $i$-th measurement, and $g_i$ is the value of $G$ on the $i$-th measurement. Intuitively, measurements have been built by choosing the repair that corresponds to the s-t tgd that best fits the ground truth. 
Consider, for example, the s-t tgd $\mu_1$ from Example~\ref{example:frepair}
and its three possible repairs $r_1$--$r_3$.
In order to compare the possibles pairs of repairs, suppose that the preference goes to the repair with the maximum number of exported variables and, 
in case of equality (i.e., $\delta_{FV} = 0$), the preference goes to the repair with the maximum number of joins.
The above leads to a training set with three measurements $\langle 1,-1,r_2\rangle$, $\langle 1,0,r_3\rangle$ and $\langle 0,1,r_3\rangle$.  
The first observation, which corresponds to the comparison between $r_1$ and $r_2$ leads to computation of values 1 and -1, choosing, thus, $r_2$; 
the second observation, which corresponds to the comparison between $r_1$ and $r_2$, leads to computation of values 1 and 0, choosing, thus, $r_3$;
the third observation, which corresponds to the comparison between $r_2$ and $r_3$, leads to computation of values 0 and 1, choosing, thus, $r_3$.

Intuitively, as shown in the previous example, the measurements 
are built by choosing the repair that corresponds to the 
s-t tgds that are the closest to the golden standard one. 
Using this training set and given an input ${\langle \delta_{FV},\delta_{J} \rangle}$, 
a predicted value $\hat{g}$ is computed with the use of the k-NN method.
More precisely, the k-NN method finds the k-nearest measurements to 
${\langle \delta_{FV,j},\delta_{J,j} \rangle}$ among the measurements of the training set.
The adopted similarity function is the Euclidean distance as further 
explained in Section \ref{sec:experiments}.
The consideration of other similarity functions as well as the adoption of other 
learning methods to learn the preference function $\pref$ fall beyond 
the scope of our paper and are deferred to future investigation. 


==> macros.tex <==
\RequirePackage{xspace}

\algdef{SE}[DOWHILE]{Do}{doWhile}{\algorithmicdo}[1]{\algorithmicwhile\ #1}

\newcommand{\angela}[1]{\textbf{Angela}: \textcolor{red}{#1}}
\newcommand{\efi}[1]{\textbf{Efi}: \textcolor{red}{#1}}
\newcommand{\ugo}[1]{{\color{red}{\modification{U}#1}}}
\newcommand{\ugoC}[2]{{\color{red}{\modification{U\ #2}#1}}}
\newcommand{\kw}[1]{{\mathsf{#1}}\xspace}

\newcommand{\vars}{\mathsf{Vars}}
\newcommand{\const}{\mathsf{Const}}
\newcommand{\nulls}{\mathsf{Nulls}}

\renewcommand*{\marginfont}{\footnotesize}
\newcommand{\circled}[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=2pt] (char) {#1};}}
\newcommand{\modification}[1]{\marginnote{\circled{\bf $\mathbf{#1}$}}[0cm]}
\newcommand{\modificationWithHeight}[2]{\marginnote{\circled{\bf $\mathbf{#2}$}}[#1]}

% \newcommand{\infacc}{\kw{InfAcc}}
% \newcommand{\canonical}{\kw{canonicalDB}}
% \newcommand{\accessiblef}{\kw{Accessible}}
% \newcommand{\accessiblefb}{\kw{Accessible^{\leftrightarrow}}}
%\newcommand{\chase}{\kw{Chase}}
% \newcommand{\monotone}{\kw{+}}
% \newcommand{\nonmonotone}{\kw{-}}
% \newcommand{\forward}{\rightarrow}
% \newcommand{\backward}{\leftarrow}
% \newcommand{\detFacts}{\kw{detFacts}}
\newcommand{\predicate}{\kw{predicate}}
\newcommand{\body}{\kw{body}}
\newcommand{\head}{\kw{head}}
\newcommand{\frontier}[1]{\kw{exported}(#1)}

\newcommand{\prem}[1]{\mathsf{premise}(#1)}
\newcommand{\dependency}[1]{\kw{dependency}(#1)}
\newcommand{\origin}[1]{\mathsf{tgd}(#1)}

% \newcommand{\facts}[1]{\mathsf{facts}(#1)}
% \newcommand{\replace}[3]{#1[#2]_{#3}}
% \newcommand{\dep}[1]{\mathsf{egd}(#1)}
% \newcommand{\egd}[1]{\mathsf{egd}(#1)}
% \newcommand{\concl}[1]{\mathsf{conclusion}(#1)}
\newcommand{\sub}[1]{\mathsf{trigger}(#1)}
\newcommand{\supp}[1]{#1^{\prec}}
\newcommand{\depth}[1]{\mathsf{depth}(#1)}
\newcommand{\myparagraph}[1]{\vspace{0.1cm}{\bf #1.}}

\newcommand{\Varb}{\mathcal{V}}
% \newcommand{\Vcan}{\mathcal{C}}
\newcommand{\Varbinstance}{V}
% \newcommand{\Vcaninstance}{C}
% \newcommand{\util}{Q}
% \newcommand{\utilsmall}{Q_{s}}
% \newcommand{\utilarb}{Q_{a}}
% \newcommand{\Vcanarb}{\mathcal{C}_{a}}
% \newcommand{\Vcansmall}{\mathcal{C}_{s}}
% \newcommand{\joinvars}{\kw{joinVariables}}
% \newcommand{\secret}{p}

\newcommand{\mappingsOriginal}{\mathcal{M}}
\newcommand{\mappingsModified}{\mathcal{M}'}
\newcommand{\mappingsInstance}{\mu}
\newcommand{\policyViews}{\mathcal{V}}
\newcommand{\policyViewInstance}{V}
\newcommand{\visibleIn}{C}
\newcommand{\instance}{I}
\newcommand{\targetInstance}{J}
\newcommand{\source}{\kw{S}}
\newcommand{\target}{\kw{T}}
\newcommand{\viewSchema}{\kw{V}}
\newcommand{\domain}{\kw{Domain}}
\newcommand{\util}{Q}
\newcommand{\secret}{p}
\newcommand{\chase}[2]{\mathsf{chase}(#1,#2)}
\newcommand{\vchase}[2]{\mathsf{visChase}_{#2}(#1)}
\newcommand{\bagchase}[2]{\mathsf{bagChase}_{#2}(#1)}
\newcommand{\indistinguishability}[3]{{#1} \equiv_{#3} {#2}}
\newcommand{\certain}[3]{\mathsf{certain}(#1,#2,#3)}
\newcommand{\inverse}[1]{#1^{-1}}
\newcommand{\critical}[1]{\mathsf{Crt}_{#1}}
\newcommand{\pos}[2]{#1|_{#2}}
\newcommand{\positions}[1]{\mathsf{pos}(#1)}
\newcommand{\dom}[1]{\mathsf{dom}(#1)}
\newcommand{\bag}{\beta}
\newcommand{\bagSet}{B}

\newcommand{\repair}{\mathsf{repair}}
\newcommand{\fphase}{\mathsf{frepair}}
\newcommand{\prov}{\mathsf{provenance}}
\newcommand{\sphase}{\mathsf{srepair}}
\newcommand{\pref}{\mathsf{prf}}
\newcommand{\hideF}{\mathsf{hideExported}}
\newcommand{\elimVars}{\mathsf{modifyBody}}
%\newcommand{\seq}{\Gamma}
\newcommand{\visins}[2]{I_{#2}(#1)}
% \newcommand{\visseq}[2]{\seq_{#2}(#1)}

\newcommand{\onc}{\mathsf{O}}
\newcommand{\pat}{\mathsf{P}}
\newcommand{\hospn}{\mathsf{H_N}}
\newcommand{\hosps}{\mathsf{H_S}}
\newcommand{\school}{\mathsf{S}}

\newcommand{\ethreason}{\mathsf{EthDis}}
\newcommand{\countyreason}{\mathsf{CountyDis}}
\newcommand{\studentOnc}{\mathsf{SO}}
\newcommand{\R}{\mathsf{R}}
\newcommand{\Sm}{\mathsf{S}}
\newcommand{\T}{\mathsf{T}}
\newcommand{\lnu}{\mathsf{n}}
\newcommand{\pid}{\mathsf{i}}
\newcommand{\name}{\mathsf{n}}
\newcommand{\ethn}{\mathsf{e}}
\newcommand{\post}{\mathsf{c}}
\newcommand{\dis}{\mathsf{d}}
\newcommand{\sid}{\mathsf{i}}
\newcommand{\tr}{\mathsf{t}}
\newcommand{\pr}{\mathsf{p}}
\newcommand{\viewPred}{\kw{V}}

% \newtheorem{theorem}{Theorem}
\newtheorem{example}{Example}
\newtheorem{claim}{Claim}
\newtheorem{conjecture}{Conjecture}
\newtheorem{property}{Property}
% \newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}
\newtheorem{resume}{Resume}
% \newtheorem{definition}{Definition}
% \newtheorem{remark}{Remark}
\newtheorem{problem}{Problem}
\newtheorem{challenge}{Challenge}
\theoremstyle{plan}

\declaretheorem[style=definition,name=Definition,qed=$\square$]{definition}
\declaretheorem[style=plain,name=Theorem,qed=$\square$]{theorem}
\declaretheorem[style=plain,name=Proposition,qed=$\square$]{proposition}
\declaretheorem[style=plain,name=Remark,qed=$\square$]{remark}

\newtheorem{op}{Open question}
\newtheorem{lemma}{Lemma}
\newtheorem{algo}{Algorithm}

\makeatletter
% Redefine the begin theorem environment to remove parentheses
\def\@Opargbegintheorem#1#2#3#4{#4\trivlist
      \item[\hskip\labelsep{#3#1}]{#3#2\@thmcounterend\ }}

\newcommand{\definerep}[2]{%
\spnewtheorem*{#1rp}{#2}{\bf}{\itshape}
\newenvironment{#1rep}[2]{%
  \ifthenelse{\equal{##1}{*}}
  {\begin{#1rp}[\ref{##2}]}
  {\begin{#1}\label{##2}}}
{\ifthenelse{\equal{\@currenvir}{#1}}{\end{#1}}{\end{#1rp}}}
}

\newcommand*{\defeq}{\mathrel{\rlap{%
    \raisebox{0.3ex}{$\m@th\cdot$}}%
    \raisebox{-0.3ex}{$\m@th\cdot$}}%
=}


==> motivation.tex <==
\section{Motivation \& Overview}\label{sec:motivation}

